A population of galaxy-scale jets discovered using LOFAR

The effects of feedback from high luminosity radio-loud AGN have been extensively discussed in the literature, but feedback from low-luminosity radio-loud AGN is less well understood. The advent of high sensitivity, high angular resolution, large field of view telescopes such as LOFAR is now allowing wide-area studies of such faint sources for the first time. Using the first data release of the LOFAR Two Metre Sky Survey (LoTSS) we report on our discovery of a population of 195 radio galaxies with 150 MHz luminosities between $3\times10^{22}$ and $1.5\times10^{25}\text{ W Hz}^{-1}$ and total radio emission no larger than 80 kpc. These objects, which we term galaxy-scale jets (GSJ), are small enough to be directly influencing the evolution of the host on galaxy scales. We report upon the typical host properties of our sample, finding that 9 per cent are hosted by spirals with the remainder being hosted by elliptical galaxies. Two of the spiral-hosted GSJ are highly unusual with low radio luminosities and FRII-like morphology. The host properties of our GSJ show that they are ordinary AGN observed at a stage in their life shortly after the radio emission has expanded beyond the central regions of the host. Based on our estimates, we find that about half of our GSJ have internal radio lobe energy within an order of magnitude of the ISM energy so that, even ignoring any possible shocks, GSJ are energetically capable of affecting the evolution of the host. The current sample of GSJ will grow in size with future releases of LoTSS and can also form the basis for further studies of feedback from low-luminosity radio sources.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
